Classical and Quantum Mechanics via Lie algebras

The goal of this book is to present classical mechanics, quantum mechanics, and statistical mechanics in an almost completely algebraic setting, thereby introducing mathematicians, physicists, and engineers to the ideas relating classical and quantum mechanics with Lie algebras and Lie groups. The book emphasizes the closeness of classical and quantum mechanics, and the material is selected in a way to make this closeness as apparent as possible. Much of the material covered here is not part of standard textbook treatments of classical or quantum mechanics (or is only superficially treated there). For physics students who want to get a broader view of the subject, this book may therefore serve as a useful complement to standard treatments of quantum mechanics. Almost without exception, this book is about precise concepts and exact results in classical mechanics, quantum mechanics, and statistical mechanics. The structural properties of mechanics are discussed independent of computational techniques for obtaining quantitatively correct numbers from the assumptions made. The standard approximation machinery for calculating from first principles explicit thermodynamic properties of materials, or explicit cross sections for high energy experiments can be found in many textbooks and is not repeated here.

==> pst-spectra.tex <==
%% BEGIN pst-spectra.tex
%%
%% This extension try to deals with wavelength in optics.
%% Beginning with spectra
%%
%% COPYRIGHT 2005,2006 by Arnaud Schmittbuhl
%%
%% This program can be redistributed and/or modified under the terms
%% of the LaTeX Project Public License Distributed from CTAN
%% archives in directory macros/latex/base/lppl.txt.
%%
\csname PSTwlLoaded\endcsname
\let\PSTwlLoaded\endinput
%
\def\pstwlfileversion{0.91}
\def\pstwlfiledate{2006/01/01}
\message{`pst-spectra'  v\pstwlfileversion, \pstwlfiledate\space (AS)}
%
% Requires pstricks, multido, pst-xkey
\ifx\PSTricksLoaded\endinput\else\input pstricks.tex\fi
\ifx\PSTXKeyLoaded\endinput\else\input pst-xkey \fi
\ifx\MultidoLoaded\endinput\else\input multido.tex\fi
%
%
\edef\TheAtCode{\the\catcode`\@}
\catcode`\@=11\relax
%
%%% Stolen code from LaTeX file: latex.ltx (coming from ltcntrl.dtx)
\def\@nnil{\@nil}
\def\@empty{}
\def\@fornoop#1\@@#2#3{}
\long\def\@for#1:=#2\do#3{%
  \expandafter\def\expandafter\@fortmp\expandafter{#2}%
  \ifx\@fortmp\@empty \else
    \expandafter\@forloop#2,\@nil,\@nil\@@#1{#3}\fi}
\long\def\@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\@nnil \else
      #5\def#4{#2}\ifx #4\@nnil \else#5\@iforloop #3\@@#4{#5}\fi\fi}
\long\def\@iforloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\@nnil
      \expandafter\@fornoop \else
      #4\relax\expandafter\@iforloop\fi#2\@@#3{#4}}
%
%
%% Prologue for postscript
\pstheader{pst-spectra.pro}
%
\SpecialCoor
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% display a continuum spectrum or lines?
%% default is spectrum
\newif\ifpst@psspectrum@spectrum \pst@psspectrum@spectrumtrue
\newif\ifpst@psspectrum@lines    \pst@psspectrum@linesfalse
\newif\ifpst@psspectrum@element  \pst@psspectrum@elementfalse
\newif\ifpst@psspectrum@emission
\newif\ifpst@psspectrum@axe
\pst@addfams{pst-wl}
\define@key[psset]{pst-wl}{begin}{\pst@checknum{#1}\psk@psspectrum@begin}
\define@key[psset]{pst-wl}{end}{\pst@checknum{#1}\psk@psspectrum@end}
\define@key[psset]{pst-wl}{axe}[true]{\@nameuse{pst@psspectrum@axe#1}}
\define@key[psset]{pst-wl}{wlangle}{\pst@checknum{#1}\psk@psspectrum@wlangle}
\define@key[psset]{pst-wl}{axecolor}{\edef\psk@psspectrum@axecolor{#1}}
%% wlcmd must be \def, not \edef
\define@key[psset]{pst-wl}{wlcmd}{\def\psk@psspectrum@wlcmd{#1}}
\define@key[psset]{pst-wl}{axewidth}{\pst@getlength{#1}\psk@psspectrum@axewidth}
\define@key[psset]{pst-wl}{Dl}{\pst@checknum{#1}\psk@psspectrum@Dl}
\define@key[psset]{pst-wl}{brightness}{\pst@checknum{#1}\psk@psspectrum@brightness}
\define@key[psset]{pst-wl}{gamma}{\pst@checknum{#1}\psk@psspectrum@gamma}
\define@key[psset]{pst-wl}{Imin}{\pst@checknum{#1}\psk@psspectrum@UserImin}
\define@key[psset]{pst-wl}{element}{\pst@psspectrum@elementtrue\edef\psk@psspectrum@element{#1}}
\define@key[psset]{pst-wl}{lines}{\pst@psspectrum@linestrue\edef\psk@psspectrum@lines{#1}}
\define@key[psset]{pst-wl}{emission}[true]{\@nameuse{pst@psspectrum@emission#1}}
\def\@temp@wl@ii{true}%
\define@key[psset]{pst-wl}{absorption}[true]%
 {\def\@temp@wl@i{#1}%
   \ifx\@temp@wl@i\@temp@wl@ii\@nameuse{pst@psspectrum@emissionfalse}%
   \else\@nameuse{pst@psspectrum@emissiontrue}%
   \fi}
\define@key[psset]{pst-wl}{lwidth}{\pst@getlength{#1}\psk@psspectrum@lwidth}
\define@key[psset]{pst-wl}{numlines}{\pst@getint{#1}\psk@psspectrum@numlines}
%\define@key[psset]{pst-wl}{showlines}{\edef\psk@psspectrum@showlines{#1}}
%\define@key[psset]{pst-wl}{redshift}{\pst@checknum{#1}\psk@psspectrum@redshift}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% default values
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\psset{begin=380, end=780, numlines=250, brightness=1, gamma=0.8, lwidth=0.02
 ,emission=true
 ,axe=false, Dl=20, wlangle=0, axecolor=black, axewidth=0.05
 ,wlcmd={\small\sffamily\bfseries}
 ,Imin=0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% code
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Scan the name of the element to know if it is a neutral element or a cation
% and to get the number of charge
% output : \element@name and \element@charge
\def\analyse@elt#1{%
  \def\analyse@elt@arg{#1}%
  \ifx\analyse@elt@arg\empty%
  \else\analyse@elt@b#1\empty\empty\empty\analyse@elt@e%
  \fi}
\def\analyse@elt@b#1#2#3#4\analyse@elt@e{%
 \gdef\element@name{}%
 \gdef\element@charge{}%
 \ifx#4\empty%
  \ifx#3\empty%
   \ifx#2\empty%
     % One letter element
     \gdef\element@name{#1}%
     \gdef\element@charge{-2}%
   \else%
    \ifx0#2%
      % Neutral one letter element
      \gdef\element@name{#1}%
      \gdef\element@charge{0}%
    \else\ifx+#2%
           % One letter single ionized element
           \gdef\element@name{#1}%
           \gdef\element@charge{1}%
         \else \ifcat#2z%
                 % Two letters element
                 \gdef\element@name{#1#2}%
                 \gdef\element@charge{-2}%
               \else % Problem
                 \@pstrickserr{Bad element or cation name: #1#2}\@ehpa
               \fi%
         \fi%
    \fi%
   \fi%
  \else%
   \ifx0#3%
     % Neutral two letters element
     \gdef\element@name{#1#2}%
     \gdef\element@charge{0}%
   \else\ifx+#3\ifcat#2z%
                  % Two letter single ionized element
                  \gdef\element@name{#1#2}%
                  \gdef\element@charge{1}%
                \else%
                  % One letter multiple ionized element
                  \gdef\element@name{#1}%
                  \gdef\element@charge{#2}%
                \fi%
        \else% Problem
          \@pstrickserr{Bad element or cation name: #1#2#3}\@ehpa
        \fi%
   \fi%
  \fi%
 \else%
 \ifx+#4%
%\ifcat1#3% <-- does not always work as expected
           % Multiple ionized two letters element
           \gdef\element@name{#1#2}%
           \gdef\element@charge{#3}%
%          \else% Problem
%          \fi%
  \else% Problem
    \@pstrickserr{Bad element or cation name: #1#2#3#4}\@ehpa
  \fi%
 \fi%
\ignorespaces}

\newdimen\pstwl@DeltaX
\newdimen\pstwl@DeltaL
\def\pst@wl@getint#1.#2\endpst@wl@getint{\def\psk@wl@int{#1}}

%% \psspectrum
\def\psspectrum{\def\pst@par{}\pst@object{psspectrum}}
\def\psspectrum@i{%
  \@ifnextchar({\psspectrum@ii}{\psspectrum@iii(0,0)(12,1.5)}}
\def\psspectrum@ii(#1){%
  \@ifnextchar({\psspectrum@iii(#1)}{\psspectrum@iii(0,0)(#1)}}
\def\psspectrum@iii(#1,#2)(#3,#4){{%
  \begin@SpecialObj
    \use@par%           Really needed ?
    \pssetxlength\pst@dima{#1}
    \pssetylength\pst@dimb{#2}
    \pssetxlength\pst@dimc{#3}
    \pssetylength\pst@dimd{#4}
    \pst@getcoor{#1,#2}\pst@tempa%            coordinate in pst@tempa
    \pst@@getcoor{#3,#4}%                      coordinate in pst@coor
    %% emission spectrum
    \ifpst@psspectrum@emission%                      emission is true
    %% ...with lines
      \ifpst@psspectrum@lines%                     drawing user lines
        \pst@psspectrum@spectrumfalse\pst@psspectrum@linesfalse
        \@for\lines@loop:=\psk@psspectrum@lines\do{%
         \addto@pscode{[[\lines@loop\space 0 -2]] 1
                        \psk@psspectrum@UserImin -2
                         \psk@psspectrum@lwidth
                          \pst@tempa \pst@coor
                           \psk@psspectrum@gamma \psk@psspectrum@brightness
                            \psk@psspectrum@end \psk@psspectrum@begin
                             tx@PstWLDict begin tx@rays end}%
        }%
      \fi
    %% ...with element
      \ifpst@psspectrum@element%            drawing lines of elements
        \pst@psspectrum@spectrumfalse\pst@psspectrum@elementfalse
         \@for\element@loop:=\psk@psspectrum@element\do{%
          \expandafter\analyse@elt\expandafter{\element@loop}
            \addto@pscode{tx@PstWLDict begin wl@elt@\element@name\space end
                           \psk@psspectrum@UserImin \element@charge\space
                            \psk@psspectrum@lwidth
                             \pst@tempa \pst@coor
                              \psk@psspectrum@gamma \psk@psspectrum@brightness
                               \psk@psspectrum@end \psk@psspectrum@begin
                                tx@PstWLDict begin tx@rays end}%
         }%
      \fi
      \ifpst@psspectrum@spectrum% drawing a spectrum
        \addto@pscode{\pst@tempa \pst@coor \psk@psspectrum@gamma
                       \psk@psspectrum@brightness \psk@psspectrum@numlines
                         \psk@psspectrum@end \psk@psspectrum@begin
                          tx@PstWLDict begin tx@psspectrum end}%
      \fi
    %% absorption spectrum
    \else% emission is false, then draw a spectrum and set brightness to 0
      \addto@pscode{\pst@tempa \pst@coor \psk@psspectrum@gamma
                     \psk@psspectrum@brightness \psk@psspectrum@numlines
                      \psk@psspectrum@end \psk@psspectrum@begin
                       tx@PstWLDict begin tx@psspectrum end}%
      \pst@checknum{0}\psk@psspectrum@brightness%
      \ifpst@psspectrum@lines% absorption lines
        \pst@psspectrum@linesfalse
        \@for\lines@loop:=\psk@psspectrum@lines\do{%
          \addto@pscode{[[\lines@loop\space 0 -2]] 1
                         \psk@psspectrum@UserImin -2
                          \psk@psspectrum@lwidth
                           \pst@tempa \pst@coor
                            \psk@psspectrum@gamma \psk@psspectrum@brightness
                             \psk@psspectrum@end \psk@psspectrum@begin
                              tx@PstWLDict begin tx@rays end}%
         }%
      \fi
      \ifpst@psspectrum@element% absorption element
        \pst@psspectrum@elementfalse
         \@for\element@loop:=\psk@psspectrum@element\do{%
          \expandafter\analyse@elt\expandafter{\element@loop}
            \addto@pscode{tx@PstWLDict begin wl@elt@\element@name\space end
                           \psk@psspectrum@UserImin \element@charge\space
                            \psk@psspectrum@lwidth
                             \pst@tempa \pst@coor
                              \psk@psspectrum@gamma \psk@psspectrum@brightness
                               \psk@psspectrum@end \psk@psspectrum@begin
                                tx@PstWLDict begin tx@rays end}%
         }%
      \fi
    \fi
    \ifpst@psspectrum@axe
      %% Calcul the number of ticks
      %% (LambdaEnd - LambdaBegin) / DL
      \pst@dimg=\z@
      \advance\pst@dimg by  \psk@psspectrum@end\p@
      \advance\pst@dimg by -\psk@psspectrum@begin\p@
      \ifnum\pst@dimg>0
        \advance\pst@dimg by \psk@psspectrum@Dl\p@
      \else
        \advance\pst@dimg by -\psk@psspectrum@Dl\p@
      \fi
      \pst@divide{\pst@dimg}{\psk@psspectrum@Dl\p@}\real@numofticks
      %% integer number of ticks is stored in \psk@wl@int
      \expandafter\pst@wl@getint\real@numofticks\endpst@wl@getint
      %% Calcul the difference between the wavelengths
      \pstwl@DeltaL=\z@
      \advance\pstwl@DeltaL by  \psk@psspectrum@end\p@
      \advance\pstwl@DeltaL by -\psk@psspectrum@begin\p@
      %% Calcul the difference between the x-coordinate
      \pstwl@DeltaX=\z@
      \advance\pstwl@DeltaX by  \pst@dimc% in pt
      \advance\pstwl@DeltaX by -\pst@dima% in pt
      %% Calcul dx
      \pst@divide{\pstwl@DeltaX}{\the\psxunit}\pst@tempa
      \pst@divide{\pstwl@DeltaL}{\pst@tempa\p@}\pst@tempb
      \pst@divide{\psk@psspectrum@Dl\p@}{\pst@tempb\p@}\dx%
      \ifdim\pst@dimd>\pst@dimb
        \def\pst@wl@angle{-90}%
        \def\pst@wl@signe{-1\space}%
      \else
        \def\pst@wl@angle{90}%
        \def\pst@wl@signe{1\space}%
      \fi
      \pst@divide{\psk@psspectrum@axewidth\p@}{28.4526\p@}\pst@tempa
      \psline[linewidth=\pst@tempa,linecolor=\psk@psspectrum@axecolor,arrows=c-c]
             (\pst@dima,\pst@dimb)(\pst@dimc,\pst@dimb)
      \edef\pst@tempb{\pst@number\pst@dima}%
      \pst@divide{\pst@tempb\p@}{\the\psxunit}\pst@tempa
      \multido{\nL=\psk@psspectrum@begin+\psk@psspectrum@Dl,\rx=\pst@tempa+\dx}
        {\psk@wl@int}%
        {\psline[linecolor=\psk@psspectrum@axecolor]
                (!\rx\space                                    % rx in cm
                 \pst@number\pst@dimb \pst@number\psyunit div) % in pt !
                (!\rx\space
                 \pst@number\pst@dimb \pst@number\psyunit div
                 0.2 \pst@wl@signe mul add)
         \uput{0.3}[\pst@wl@angle]
              (!\rx\space
               \pst@number\pst@dimb \pst@number\psyunit div
               0.1 \pst@wl@signe mul add)
              {\rput{\psk@psspectrum@wlangle}{\psk@psspectrum@wlcmd\nL}}}%
    \fi
    \pst@psspectrum@spectrumtrue
  \end@SpecialObj
}}%

\catcode`\@=\PstAtCode\relax
\endinput
%% END pst-spectra.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

